AffectNet+: A Database for Enhancing Facial Expression Recognition with Soft-Labels

Automated Facial Expression Recognition (FER) is challenging due to intra-class variations and inter-class similarities. FER can be especially difficult when facial expressions reflect a mixture of various emotions (aka compound expressions). Existing FER datasets, such as AffectNet, provide discrete emotion labels (hard-labels), where a single category of emotion is assigned to an expression. To alleviate inter- and intra-class challenges, as well as provide a better facial expression descriptor, we propose a new approach to create FER datasets through a labeling method in which an image is labeled with more than one emotion (called soft-labels), each with different confidences. Specifically, we introduce the notion of soft-labels for facial expression datasets, a new approach to affective computing for more realistic recognition of facial expressions. To achieve this goal, we propose a novel methodology to accurately calculate soft-labels: a vector representing the extent to which multiple categories of emotion are simultaneously present within a single facial expression. Finding smoother decision boundaries, enabling multi-labeling, and mitigating bias and imbalanced data are some of the advantages of our proposed method. Building upon AffectNet, we introduce AffectNet+, the next-generation facial expression dataset. This dataset contains soft-labels, three categories of data complexity subsets, and additional metadata such as age, gender, ethnicity, head pose, facial landmarks, valence, and arousal. AffectNet+ will be made publicly accessible to researchers.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tbls/annotator_dist.tex <==
\begin{table}[] 
\caption{The correspondence between the number of annotators and images in the \textit{gold-set}.}
\label{tbl:annotator_dist}
\centering
\small
\resizebox{0.48\textwidth}{!}
{{
\begin{tabular}{lcccc}
\hline
\textbf{\# Annotators} & Two   & Three & Four & Five \\ 
\textbf{\# Images}     & 32378 & 2373  & 997  & 302  \\ \hline
\end{tabular}
}}
\end{table}

==> tbls/efficientnet_hard_label_accuracy.tex <==
\begin{table}[t!] 
\caption{Accuracy on different sets of AffectNet+ on the EfficientNet-B3\cite{tan2019efficientnet}.}
\label{tbl:efficientnet_hard_label_accuracy}
\centering
\small
\resizebox{0.48\textwidth}{!}
{{
\begin{tabular}{lcccc}
\hline
        & All   & Normal & Challenging & Hard  \\ \hline
Acc (\%)     & 55.17 & 87.06  & 57.13       & 41.25 \\
$\overline{Acc}$ (\%) & 55.13 & 81.44  & 55.71       & 42.36 \\ \hline
\end{tabular}}}
\end{table}

==> tbls/efficientnet_hard_label_prec_rec_f1.tex <==
\begin{table}[t!] 
\caption{Precision, recall, and f-1 score on different sets of AffectNet+, using the EfficientNet-B3\cite{tan2019efficientnet} model (in \%).}
\label{tbl:efficientnet_hard_label_prec_rec_f1}
\centering
\small
\resizebox{0.48\textwidth}{!}
{{
\begin{tabular}{lcccccccc}
\hline
     & Neutral & Happy & Sad   & Surprise & Anger & Disgust & Fear  & Contempt \\ \hline
     & \multicolumn{8}{c}{All}                                                 \\ \hdashline
Prec & 39.35   & 56.89 & 57.83 & 55.64    & 76.41 & 81.30   & 48.64 & 75.69    \\
Rec  & 66.73   & 85.34 & 62.50 & 53.73    & 46.84 & 35.15   & 68.68 & 22.06    \\
F-1  & 49.51   & 68.27 & 60.07 & 54.67    & 58.08 & 49.08   & 56.95 & 34.16    \\ \hline
     & \multicolumn{8}{c}{Normal}                                              \\ \hdashline
Prec & 86.64   & 96.83 & 67.12 & 91.40    & 86.02 & 92.47   & 86.95 & 68.42    \\
Rec  & 86.13   & 97.49 & 91.87 & 79.05    & 88.63 & 71.07   & 85.30 & 52.00    \\
F-1  & 86.39   & 97.16 & 77.57 & 84.78    & 87.31 & 80.37   & 86.12 & 59.09    \\ \hline
     & \multicolumn{8}{c}{Challenging}                                         \\ \hdashline
Prec & 27.18   & 11.39 & 62.22 & 62.08    & 77.69 & 63.88   & 55.41 & 80.42    \\
Rec  & 31.46   & 56.25 & 66.98 & 65.31    & 59.76 & 63.88   & 52.40 & 49.67    \\
F-1  & 29.16   & 18.94 & 64.51 & 63.66    & 67.55 & 63.88   & 53.86 & 61.41    \\ \hline
     & \multicolumn{8}{c}{Hard}                                                \\ \hdashline
Prec & 24.64   & 16.32 & 35.86 & 44.63    & 67.82 & 43.63   & 31.44 & 73.01    \\
Rec  & 55.55   & 42.10 & 42.97 & 46.74    & 41.71 & 31.57   & 44.64 & 33.57    \\
F-1  & 34.14   & 23.52 & 39.09 & 45.66    & 51.65 & 36.64   & 36.90 & 46.00    \\ \hline
\end{tabular}
}}
\end{table}

==> tbls/efficientnet_soft_label_error.tex <==
\begin{table}[t!] 
\caption{Error on different sets of AffectNet+ on EfficientNet-B3\cite{tan2019efficientnet}.}
\label{tbl:efficientnet_soft_label_error}
\centering
\small
\resizebox{0.35\textwidth}{!}
{{
\begin{tabular}{lcccc}
\hline
                    & All       & Normal    & Challenging & Hard  \\ \hline
W-FR (\%)           & 10.58     & 6.28      & 11.25       & 18.35 \\
W-MAE (\%)          & 17.03     & 15.13     & 18.63        & 20.81  \\
% $\text{W-AUC}_{\epsilon}$                & ? & ?  & ?       & ? \\ 
\hline
\end{tabular}}}
\end{table}

==> tbls/efficientnet_soft_label_error_on_expression.tex <==
\begin{table}[t!] 
\caption{Failure rate, mean average error, and AUC on soft labels, based on the EfficientNet-B3 \cite{tan2019efficientnet} model, on different expressions.}
\label{tbl:efficientnet_soft_label_error_on_expression}
\centering
\small
\resizebox{0.48\textwidth}{!}
{{
\begin{tabular}{llcccc}
\hline
                          &     & All   & Normal & Challenging & Hard  \\ \hline
\multirow{3}{*}{Neutral}  & FR  & 11.00 & 4.66   & 20.00       & 20.90 \\
                          & MAE & 17.24 & 15.09  & 22.00       & 22.42 \\
                          % & AUC &       &        &             &       \\ 
                          \hdashline
\multirow{3}{*}{Happy}    & FR  & 3.40  & 1.34   & 6.25        & 19.05 \\
                          & MAE & 11.98 & 10.79  & 18.27       & 23.02 \\
                          % & AUC &       &        &             &       \\ 
                          \hdashline
\multirow{3}{*}{Sad}      & FR  & 11.80 & 6.06   & 9.05        & 16.80 \\
                          & MAE & 17.88 & 17.62  & 17.47       & 19.64 \\
                          % & AUC &       &        &             &       \\ 
                          \hdashline
\multirow{3}{*}{Surprise} & FR  & 12.20 & 11.49  & 14.20       & 18.75 \\
                          & MAE & 17.77 & 17.20  & 19.17       & 20.41 \\
                          % & AUC &       &        &             &       \\ 
                          \hdashline
\multirow{3}{*}{Fear}     & FR  & 14.80 & 11.19  & 15.20       & 19.49 \\
                          & MAE & 18.74 & 17.81  & 19.18       & 21.75 \\
                          % & AUC &       &        &             &       \\
                          \hdashline
\multirow{3}{*}{Disgust}  & FR  & 12.40 & 13.01  & 10.91       & 19.11 \\
                          & MAE & 18.27 & 17.56  & 19.08       & 21.58 \\
                          % & AUC &       &        &             &       \\ 
                          \hdashline
\multirow{3}{*}{Anger}    & FR  & 11.60 & 9.35   & 11.18       & 13.79 \\
                          & MAE & 17.90 & 16.92  & 19.23       & 19.73 \\
                          % & AUC &       &        &             &       \\ 
                          \hdashline
\multirow{3}{*}{Contempt} & FR  & 7.40  & 3.92   & 7.12        & 19.29 \\
                          & MAE & 16.45 & 18.90  & 17.22       & 20.00 \\
                          % & AUC &       &        &             &       \\
                          \hline
\end{tabular}
}}
\end{table}



==> tbls/ensemble_of_binary_classifiers_and_action_units_on_test_MAS.tex <==
\begin{table}[b] 
\caption{Accuracy over each expression, using the ensemble of binary classifier and action unit-based models over test-MAS (in \%).}
\label{tbl:ensemble_eval_test_MAS}
\centering
\small
\resizebox{0.48\textwidth}{!}
{{
\begin{tabular}{lcccccccc}
\hline
 & Neutral & Happy & Sad   & Surprise & Fear & Disgust & Anger & Contempt \\ \hline
Acc     & 84.8    & 83.4  & 87.4  & 88.3     & 91.3 & 91.0    & 83.1  & 86.7     \\
$\overline{Acc}$ & 88.7    & 87.5  & 84.6  & 90.7     & 89.0 & 86.3    & 84.8  & 77.8     \\ \hline
\end{tabular}
}}
\end{table}

==> tbls/fer_accuracy.tex <==
\begin{table}[t!] 
\caption{Some of the most recent FER accuracies on different datasets.}
\label{tbl:fer_accuracy}
\centering
\small
\resizebox{0.48\textwidth}{!}
{{
\begin{tabular}{lccc}
\hline
work                                            & Year          & Dataset            & Accuracy(\%) \\ 
\hline
Zhu et al.\cite{zhu2022convolutional}           & 2022          & FER-2013            & 67.32             \\
Cai et al.\cite{cai2022probabilistic}           & 2022          & FER-2013            & 73.28             \\
Ma et al.\cite{ma2022multi}                     & 2022          & RAF-DB              & 64.31             \\
Xu et al.\cite{xu2020investigating}             & 2020          & RAF-DB              & 74.80             \\
Arnaud et al.\cite{arnaud2022thin}              & 2022          & ExpW                & 76.08             \\
Cai et al.\cite{cai2022probabilistic}           & 2022          & ExpW                & 72.93             \\
Zhao et al.\cite{zhao2022spatial}               & 2022          & Oulu-CASIA          & 89.17             \\
Zou et al.\cite{zou2022new}                     & 2022          & Oulu-CASIA          & 96.51             \\
Zhu et al.\cite{zhu2022convolutional}           & 2022          & SFEW                & 54.87             \\
Savchenko et al.\cite{savchenko2022classifying} & 2022          & AFEW                & 65.50              \\
Bisogni et al.\cite{bisogni2022impact}          & 2022          & CK+                 & 97.83             \\
Sun et al.\cite{sun2023discriminatively}	    & 2023	        & KDEF	              & 98.30	            \\
Sun et al.\cite{sun2023discriminatively}	    & 2023	        & JAFFE	              & 98.37	            \\
Ma et al.\cite{ma2022multi}                     & 2022          & FER+                & 66.43             \\
Liu et al.\cite{liu2022clip}                    & 2022          & MMI                 & 91.00               \\
Zhao et al.\cite{zhao2022spatial}               & 2022          & eNTERFACE05         & 54.62             \\
Xue et al.\cite{xue2022coarse}                  & 2022          & Aff-Wild2           & 32.17             \\
Kuruvayil et al.\cite{kuruvayil2022emotion}     & 2022          & MultiPie            & 90.00             \\
Tan et al.\cite{tan2022emotion}                 & 2022          & DISFA               & 95.91             \\
Borgalli and Surve\cite{borgalli2022deep}       & 2022          & AM-FED+             & 54.13             \\
Cao et al.\cite{cao2020e2}                      & 2020          & EmotioNet           & 55.91             \\
Kartheek et al.\cite{kartheek2022windmill}      & 2022          & FERG                & 99.74             \\
Rao et al.\cite{rao2020recognition}             & 2020          & DAiSEE              & 54.42             \\
\hline 
\end{tabular}
}}
\end{table}

==> tbls/fer_accuracy_on_affectnet.tex <==
\begin{table}[t!] 
\caption{FER accuracy on AffectNet.}
\label{tbl:fer_accuracy_on_affectnet}
\centering
\small
\resizebox{0.48\textwidth}{!}
{{
\begin{tabular}{lccc}
\hline
Work                                    & Year                  & \# Exp & Accuracy (\%)\\
\hline
Gong et al. \cite{gong2023mpcsan}                   & 2023                  & 8       & 61.58       \\
Liu et al. \cite{liu2023joint}                     & 2023                  & 8       & 56.80       \\
Gao et al. \cite{gao2023ssa}                       & 2023                  & 7       & 65.78       \\

Fard et al. \cite{fard2022ad}                & 2022          & 7                         & 63.36    \\
Arnaud et al.\cite{arnaud2022thin}              & 2022          & 7         & 63.79             \\

Zhang et al. \cite{zhang2022improving}               & 2022                  & 7       & 62.10       \\
Gera et al. \cite{gera2022cern}                     & 2022                  & 7       & 62.06       \\
Lang et al. \cite{lang2022multi}   & 2022 & 7       & 66.56       \\
Lang et al.\cite{lang2022multi}   & 2022 & 8       & 63.30       \\
Ma et al. \cite{ma2022relation}  & 2022 & 7       & 65.65       \\
Ma et al. \cite{ma2022relation}  & 2022 & 8       & 61.14       \\
Kuruvayil et al. \cite{kuruvayil2022emotion}             & 2022                  & 5       & 68.00       \\
Zeng et al. \cite{zeng2022face2exp}                 & 2022                  & 7       & 64.23       \\
Liu et al. \cite{liu2022uncertain}                 & 2022                  & 7       & 61.57       \\
Zheng et al. \cite{zheng2022poster} & 2022 & 7       & 67.31       \\
Zheng et al. \cite{zheng2022poster} & 2022 & 8       & 63.34       \\
Su et al. \cite{su2022using}                      & 2022                  & 8       & 58.68       \\
Heidari et al. \cite{heidari2022learning}              & 2022                  & 8       & 60.02       \\
Wang et al. \cite{wang2022bias}    & 2022 & 7       & 64.45       \\
Wang et al. \cite{wang2022bias}    & 2022 & 8       & 60.24       \\
Jiang et al. \cite{jiang2021boosting}   & 2021                  & 8       & 58.54       \\

\hline
\end{tabular}
}}
\end{table}

==> tbls/fer_datasets.tex <==
\begin{table}[t!] 
\caption{Some of the datasets in affect computing. The symbols are as follow: I$\rightarrow$Image, VS$\rightarrow$Video Sequence, AU$\rightarrow$Action Unit, C$\rightarrow$Controlled, P$\rightarrow$Posed, S$\rightarrow$Spontaneous, W$\rightarrow$Wild, V$\rightarrow$Valence, A$\rightarrow$Arousal, MD$\rightarrow$Meta-Data, MA$\rightarrow$Manually Annotated, AA$\rightarrow$Automatically (Machine) Annotated, NIR$\rightarrow$Near Infrared, D$\rightarrow$Dimension, K$\rightarrow$Kilo.}
\label{tbl:fer_datasets}
\centering
\small
\resizebox{0.48\textwidth}{!}
{
\begin{tabular}{ll}
\hline
Name & Attributes \\
\hline
AffectNet\cite{mollahosseini2017affectnet} & I: $\sim$1M, Exp: 8, W, V, A, MD, MA: $\sim$440K \\ 
RAF-DB\cite{li2017reliable} & I: $\sim$30K, Exp: 7, W, MD  \\
CK+\cite{lucey2010extended} & VS: 593, Exp: 7, C, P, AU: 30, MA: 327  \\
Aff-Wild\cite{zafeiriou2016facial} & VS: 500, I: 10K, AU: 16, S, W, V, A  \\
Aff-Wild2\cite{kollias2018aff} & Aff-Wild + VS: 260, W, V, A \\
FER-Wild\cite{mollahosseini2016facial} & I: $\sim$120K, Exp: 7, W, MD, MA: 24K  \\
MultiPie\cite{GROSS2010807} & I: $\sim$750K, Exp: 6, C, P  \\
MMI\cite{pantic2005web} & VS + I: $\sim$1.5K, Exp: 6, AU: 31, C, P, MD \\
DISFA\cite{mavadati2013disfa} & VS: 27, AU: 12, C, S, MD \\
RECOLA\cite{ringeval2013introducing} & VS: 46, Exp: 5, S, V, A, MD \\
AM-FED\cite{mcduff2013affectiva} & VS: 242, AU: 16, S, MD \\
DEAP\cite{koelstra2011deap} & VS: 32, C, S, V, A, MD  \\
AFEW\cite{dhall2012collecting} & VS:1426, Exp:7, W, MD \\
SFEW\cite{dhall2011static} & I: 700, Exp: 7, W, MD  \\
FER-2013\cite{goodfellow2013challenges} & I: $\sim$36K, Exp:7, W \\
EmotioNet\cite{fabian2016emotionet} & I: 1M, Exp: 23, AU: 15, W, not AA \\
FERG\cite{aneja2017modeling} & I: $\sim$56K, Exp: 7, Synthesized Cartoon Images  \\
Oulu-CASIA\cite{zhao2011facial} & I: $\sim$3K, Exp: 6, C, P, NIR \\
AR Face\cite{martinez1998ar} & I: $\sim$4K, Exp: 4, C, P \\
JAFFE\cite{lyons1998coding} & I: 219, Exp: 7, C, P, Japanese Females \\
GFT\cite{girard2017sayette} & VS: 96, AU: 20, C, S \\
B4PD\cite{zhang2013high} & VS: 41, Exp: 6, AU: 32, C, S, MD, 2D/3D \\
B4PD+\cite{zhang2016multimodal} & VS:140, AU: 32, C, S, MD, 2D/3D, NIR\\
4DFAB\cite{cheng20184dfab} & I: 1.8M Mesh, Exp: 6, P, S, MD, 3D/4D  \\
Belfast\cite{sneddon2011belfast} & VS: 1400, Exp: 3-5-7, C, S, V, MD \\
DAiSEE\cite{gupta2016daisee} & VS: $\sim$9K, Exp: 4, W, Multi-Label \\
FER+\cite{BarsoumICMI2016} & I: $\sim$36K, Exp: 7, W, Multi-Annotator \\
ExpW\cite{zhang2018facial} & I: $\sim$90K, Exp: 7, W \\
FEAFA+\cite{gan2022feafa+} & VS: 150, AU: 24, C, P, S, W  \\
KDEF\cite{lundqvist1998karolinska} & I: 490, Exp: 7, C, P, A \\
\hline
\end{tabular}}
\end{table}


==> tbls/subset_distribution_validation_set.tex <==
\begin{table}[t!] 
\caption{Per class distribution of validation set and its subsets.}
\label{tbl:subset_distribution_validation_set}
\centering
\small
\resizebox{0.48\textwidth}{!}
{{

\begin{tabular}{lcccccccc}
\hline 
& Neutral  & Happy  & Sad   & Surprise & Anger & Disgust & Fear  & Contempt                      \\ \hline
All         & 500 & 500 & 500 & 500 & 500 & 500 & 500 & 500      \\ \hdashline
Normal      
& \begin{tabular}[c]{@{}c@{}}    343    \\ (68.60\%)    \end{tabular}
& \begin{tabular}[c]{@{}c@{}}    447    \\ (89.40\%)    \end{tabular} 
& \begin{tabular}[c]{@{}c@{}}    165    \\ (33.00\%)    \end{tabular}  
& \begin{tabular}[c]{@{}c@{}}    148    \\ (29.60\%)    \end{tabular} 
& \begin{tabular}[c]{@{}c@{}}    134    \\ (26.80\%)    \end{tabular} 
& \begin{tabular}[c]{@{}c@{}}    123    \\ (24.60\%)    \end{tabular}   
& \begin{tabular}[c]{@{}c@{}}    214    \\ (42.80\%)    \end{tabular} 
& \begin{tabular}[c]{@{}c@{}}    51     \\ (10.20\%)    \end{tabular}    \\ \hdashline

Challenging 
& \begin{tabular}[c]{@{}c@{}}    90     \\ (18.00\%)\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}    32     \\ (6.40\%)\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}    210    \\ (42.00\%)\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}    176    \\ (35.20\%)\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}    171    \\ (34.20\%)\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}    220    \\ (44.00\%)\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}    170    \\ (34.00\%)\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}    309    \\ (61.80\%)\end{tabular} \\ \hdashline
Hard        
& \begin{tabular}[c]{@{}c@{}}    67    \\ (13.40\%)\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}    21    \\ (4.20\%)\end{tabular}    
& \begin{tabular}[c]{@{}c@{}}    125   \\ (25.00\%)\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}    176   \\ (35.20\%)\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}    195   \\ (39.00\%)\end{tabular}
& \begin{tabular}[c]{@{}c@{}}    157   \\ (31.40\%)\end{tabular}
& \begin{tabular}[c]{@{}c@{}}    116   \\ (23.20\%)\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}    140   \\ (28.00\%)\end{tabular}    
\\ 
\hline
\end{tabular}}}
\end{table}
